Teaching Visual Accessibility in Introductory Data Science Classes with Multi-Modal Data Representations

Although there are various ways to represent data patterns and models, visualization has been primarily taught in many data science courses for its efficiency. Such vision-dependent output may cause critical barriers against those who are blind and visually impaired and people with learning disabilities. We argue that instructors need to teach multiple data representation methods so that all students can produce data products that are more accessible. In this paper, we argue that accessibility should be taught as early as the introductory course as part of the data science curriculum so that regardless of whether learners major in data science or not, they can have foundational exposure to accessibility. As data science educators who teach accessibility as part of our lower-division courses in two different institutions, we share specific examples that can be utilized by other data science instructors.

==> header-hidden.tex <==
% For anonymity
\newcommand{\repo}[1]{HIDDEN FOR REVIEW}
\newcommand{\audio}[1]{HIDDEN FOR REVIEW}
\newcommand{\video}[1]{HIDDEN FOR REVIEW}

% Remove green borders around links
\usepackage{xcolor}
\xdefinecolor{blue}{rgb}{0.28,0.65,0.9}
\hypersetup{
    colorlinks,
    linkcolor={blue},
    citecolor={blue},
    urlcolor={blue}
}

==> header.tex <==
\usepackage{hyperref}

% For anonymity
\newcommand{\repo}[1]{https://github.com/jooyoungseo/teaching-accessibility-manuscript}
\newcommand{\audio}[1]{https://jooyoungseo.github.io/teaching-accessibility-manuscript/audio/sonify-example.wav}
\newcommand{\video}[1]{https://www.youtube.com/watch?v=ClI555l4Z1M&ab_channel=JooYoungSeo}


% Remove green borders around links
\usepackage{xcolor}
\xdefinecolor{blue}{rgb}{0.28,0.65,0.9}
\hypersetup{
    colorlinks,
    linkcolor={blue},
    citecolor={blue},
    urlcolor={blue}
}
